Solving Gossip Problems using Answer Set Programming: An Epistemic Planning Approach

We investigate the use of Answer Set Programming to solve variations of gossip problems, by modeling them as epistemic planning problems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{52}
\providecommand{\publicationstatus}{F. Ricca, A. Russo et al. (Eds.): Proc.\ 36th International Conference \\
on Logic Programming (Technical Communications) 2020 (ICLP 2020)\\
EPTCS 325, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.325.11}{10.4204/EPTCS.325.11}}
\pdfoutput=1

